Beat the long tail: Distribution-Aware Speculative Decoding for RL Training

Reinforcement learning(RL) post-training has become essential for aligning large language models (LLMs), yet its efficiency is increasingly constrained by the rollout phase, where long trajectories are generated token by token. We identify a major bottleneck:the long-tail distribution of rollout lengths, where a small fraction of long generations dominates wall clock time and a complementary opportunity; the availability of historical rollouts that reveal stable prompt level patterns across training epochs. Motivated by these observations, we propose DAS, a Distribution Aware Speculative decoding framework that accelerates RL rollouts without altering model outputs. DAS integrates two key ideas: an adaptive, nonparametric drafter built from recent rollouts using an incrementally maintained suffix tree, and a length aware speculation policy that allocates more aggressive draft budgets to long trajectories that dominate makespan. This design exploits rollout history to sustain acceptance while balancing base and token level costs during decoding. Experiments on math and code reasoning tasks show that DAS reduces rollout time up to 50% while preserving identical training curves, demonstrating that distribution-aware speculative decoding can significantly accelerate RL post training without compromising learning quality.

==> _s1_intro.tex <==
\section{Introduction}

\label{sec:intro}

Reinforcement learning (RL) has emerged as a cornerstone of large language model (LLM) post-training. By directly optimizing for desired behaviors, RL enables models to align with human preferences and verifiable objectives through reward signals derived from task-specific feedback~\citep{ouyang2022training,bai2022constitutionalaiharmlessnessai}. This approach has proven especially effective in domains such as mathematics and programming, where correctness can be automatically verified via unit tests, proof checkers, or reference outputs.


Building on the momentum of recent large-scale RL systems such as DeepSeek-R1~\citep{guo2025deepseek} and VeRL~\citep{sheng2024hybridflow}, researchers have continued to scale up RL training pipelines. However, as the size of models and datasets grow, the generation (rollout) phase
has become the dominant bottleneck in wall-clock time. Profiling studies show that rollout computation now accounts for more than 70\%~\cite{verl_one_step_off_2024} of the total training time, often exceeding the cost of backpropagation and parameter updates. The rollout phase cost can further be increased by scaling the number of samples~\citep{wang2025reinforcement}. This imbalance arises from two key factors: (1) increasing task complexity drives longer generations, and (2) the inherently autoregressive nature of decoding limits parallelism, creating a severe throughput bottleneck. 

Despite this growing bottleneck, most existing systems are not designed with rollout efficiency as the primary concern. Many RL training pipelines still assume that the optimization or backpropagation phase remains the dominant bottleneck, and thus allocate system resources accordingly~\cite{rlhfuse_2025}. Other systems emphasize inference-time throughput optimizations, such as decoupling prefill and decode to improve hardware utilization~\citep{zhong2024distserve}. While these designs increase request-level throughput, they do not address the fundamental inefficiencies of large-scale rollout collection, since all rollouts must complete before the next training phase can proceed. A separate line of work accelerates rollouts by relaxing training fidelity constraints—for instance, through truncation or quantization strategies~\cite{zhong2025streamrlscalableheterogeneouselastic}. These methods can reduce latency but often compromise learning stability or degrade performance on reasoning-heavy tasks where long-horizon rollouts are essential.


% Given this growing bottleneck, recent work has focused on system-level approaches to accelerate rollouts primarily on throughput. Disaggregating prefill and decode improves utilization and reduces head-of-line blocking, but it does not eliminate the long-tail effect where a few lengthy generations stall the batch~\citep{zhong2024distserve, zhong2025streamrlscalableheterogeneouselastic}. Similarly, truncation heuristics can reduce latency but risk degrading training quality on reasoning-heavy tasks. 


% Skewness-aware data dispatching mitigates inter-request skewness by grouping similar-length requests, but it relies on accurate length prediction—an error in even one request can reintroduce severe intra-batch skewness and fail to address intra-request imbalance.  Consequently, batch-size skew—where a handful of long rollouts dictate step time—remains a major efficiency barrier.

% To accelerate generation, a natural idea is to employ **speculative decoding**~\citep{leviathan2023fastspec}, which predicts multiple draft tokens in parallel and verifies them efficiently. Yet applying this technique to RL training introduces unique challenges. RL rollouts are conducted under rapidly evolving policy parameters, making it difficult to maintain a reliable draft model: once the policy updates, previously trained speculative decoders quickly become stale and lose acceptance efficiency.

% In this work, we present a novel **suffix-tree–based speculative decoding framework** tailored for RL post-training. Our key insight is that RL training repeatedly revisits the same dataset across epochs, creating opportunities to leverage past rollouts as a source of predictive structure. By dynamically updating a suffix-tree representation of historical generations, we can provide accurate token-level drafts that adapt as the policy evolves—without maintaining a separate neural draft model. This approach simultaneously alleviates batch-size skew and accelerates long-tail generations by reusing historical computation.

% Through experiments spanning mathematical reasoning, code generation, and tool-use tasks, our method consistently achieves up to 2× faster rollouts and substantial wall-clock reductions while preserving training stability and final reward performance. Our contributions are summarized as follows:

A natural direction is speculative decoding~\citep{leviathan2023fastspec} (SD), which proposes multiple draft tokens and verifies them with the target model. However, applying speculation naively to RL training raises two problems. First, the policy parameters evolve rapidly during training; fixed draft models quickly become stale, sharply reducing acceptance rates and eroding speedups. Second, given the large trajectory datasets needed for a training step, rollouts are typically conducted with large batches to amortize overheads. However, previous work about speculative decoding in throughput-oriented scenarios focuses more on online serving systems. They cannot fully utilize the unique characteristics of RL post-training, so the solution falls into the local maximum.

% We introduce xxx framework that adapts speculative decoding to speedup of RL training. 

% Our key insight is to mine historical rollouts from repeated passes over the fixed dataset to construct an online suffix-structure (e.g., suffix tree/DAWG/trie) that serves as a non-parametric draft generator. We update this structure continuously as training progresses, maintaining draft reliability without training a separate neural draft model. In parallel, we schedule speculation opportunistically to soak up idle compute created by batch skew: short rollouts and completed samples donate GPU headroom to speculative verification for stragglers, improving end-to-end goodput without impacting synchronous step semantics.

% \begin{itemize}
% % \item We propose a new metric: total generation step for rollout performance 
% \item We provide key insights and models about how to optimize RL training 
% \item We propose a variant of suffix decoding to optimize the RL traning. 
% \item We propose a 
% \item We epxierment different strategy to dynamic update the suffix tree to 
% \item We demonstrate that our approach reduces rollout cost by up to ?× while maintaining comparable training quality across diverse reasoning tasks.
% \end{itemize}

% \todo{some summaries}
To circumvent these failure modes, we present \textbf{\Ours, an RL training framework that integrates speculative decoding.} 
% \todo{clause about the benefits of \Ours}

We begin by theoretically and experimentally analyzing the bottlenecks of RL training and provide actionable guidance for optimization, identifying longtail generations as the principle source of overhead. Next, we discuss the approach underlying \Ours: instead of relying on a static learned drafter, we introduce a \emph{training-free, self-evolved} drafter based on an incrementally maintained suffix tree representation of recent rollouts. More importantly, we propose a distribution-aware speculative decoding, which allocates draft budget preferentially to high-difficulty, long-horizon prompts, those that dominate the rollout makespan rather than speculating uniformly.

%% OLD VERSION: 
% todo: some summaries We first theoretically and experimen-
% tally analyze the bottlenecks of RL training and provide
% actionable guidance for optimization, identifying ??? as the
% principal source of overhead.
% Next, we introduce an RL training framework that inte-
% grates speculative decoding with a suffix tree-based repre-
% sentation (Weiner, 1973; Oliaro et al., 2025). We develop
% improved construction and update procedures for the tree to
% , thereby . (todo: few sentence about the tree construction
% and update).

% We adopt a suffix-decoding–based accuracy preservation approach to improve rollout performance. 

Our framework incorporates the following contributions: 

1. \emph{Length-aware speculative decoding:} We propose a dynamic draft-allocation strategy that leverages rollout statistics to schedule speculation asymmetrically across long and short generations, reducing wasted computation while collapsing the long-tail latency.

2. \emph{Speculative decoding with history-awareness:} As RL training progresses, the policy distribution evolves over time. To remain aligned with the current policy, we prune the suffix structure dynamically, retaining only recent and relevant historical rollouts for improved locality and reliability.

3. \emph{Task-specific suffix structures:} Instead of maintaining a single global suffix tree, we construct and update per-problem trees. This design better captures domain-specific patterns and improves the accuracy of speculation in heterogeneous tasks.

Our experiments show that \Ours{} reduces rollout time by over 30\% while replicating the original training curve, indicating no loss in learning quality.


==> _s3_method.tex <==
\section{Method}
\subsection{Drafter}
\subsubsection{Rationale}
\paragraph{Generation trajectory similarity}
(i) during training, generation trajectories become similar
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/generation_sim.png}
    \caption{dummy figure from other paper to show similarity, need to change to our data}
    \label{fig:heatmap}
\end{figure}

(ii) Similarity pattern
\begin{figure}[H]
    \centering
    % ---- 子图 (a) ----
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/pairwise_similarity.png}
        \label{fig:qwen7b}
    \end{subfigure}
    \hfill
\end{figure}

\paragraph{}
\subsubsection{Design}
\subsection{Draft Budgeting Strategy}
\subsubsection{Rationale}
